SAMwave: Wavelet-Driven Feature Enrichment for Effective Adaptation of Segment Anything Model

The emergence of large foundation models has propelled significant advances in various domains. The Segment Anything Model (SAM), a leading model for image segmentation, exemplifies these advances, outperforming traditional methods. However, such foundation models often suffer from performance degradation when applied to complex tasks for which they are not trained. Existing methods typically employ adapter-based fine-tuning strategies to adapt SAM for tasks and leverage high-frequency features extracted from the Fourier domain. However, Our analysis reveals that these approaches offer limited benefits due to constraints in their feature extraction techniques. To overcome this, we propose \textbf{\textit{SAMwave}}, a novel and interpretable approach that utilizes the wavelet transform to extract richer, multi-scale high-frequency features from input data. Extending this, we introduce complex-valued adapters capable of capturing complex-valued spatial-frequency information via complex wavelet transforms. By adaptively integrating these wavelet coefficients, SAMwave enables SAM's encoder to capture information more relevant for dense prediction. Empirical evaluations on four challenging low-level vision tasks demonstrate that SAMwave significantly outperforms existing adaptation methods. This superior performance is consistent across both the SAM and SAM2 backbones and holds for both real and complex-valued adapter variants, highlighting the efficiency, flexibility, and interpretability of our proposed method for adapting segment anything models.

==> Tables/blur.tex <==
\begin{table*}[h]
\centering
\caption{Comparison with state-of-the-art approaches on defocus blur detection. The best result is shown in \textbf{bold}, and the second best is \underline{underlined}.}
 \label{tab:blur}
        \setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1}
        \resizebox{.5\linewidth}{!}{
      
      \centering
        \begin{tabular}{lcc|cc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c|}{DUT} & \multicolumn{2}{c}{CUHK} \\
                                & $\mathcal{F}_{\beta} \uparrow$    & $\mathcal{M} \downarrow$   & $\mathcal{F}_{\beta} \uparrow$    & $\mathcal{M} \downarrow$ \\ \midrule
          DeFusionNet$^{(2019)}$\cite{DBLP:conf/cvpr/TangZLWZ19}                      & 0.823      & 0.118     & 0.818      & 0.117     \\
          BTBNet$^{(2018)}$\cite{DBLP:conf/cvpr/ZhaoZ0L18}                      & 0.827      & 0.138     & 0.889      & 0.082     \\
          CENet$^{(2019)}$\cite{DBLP:conf/cvpr/ZhaoZLL19}                      & 0.817      & 0.135     & 0.906      & 0.059     \\
          DAD$^{(2021)}$ \cite{DBLP:conf/cvpr/ZhaoSL21}                     & 0.794      & 0.153     & 0.884      & 0.079     \\
          EFENet$^{(2021)}$\cite{DBLP:journals/tip/ZhaoHHL21}                      & 0.854      & 0.094     & 0.914      & 0.053     \\
          EVP$^{(2023)}$\cite{DBLP:conf/cvpr/LiuSPC23}                      & 0.890      & {0.068}     & \textbf{0.928}      & {0.045}     \\ 
    \midrule
    \multicolumn{5}{c}{SAM as backbone}\\
    \midrule
    \multicolumn{5}{l}{\textbf{Real-valued Adapters}} \\ 
    \midrule
          Ours (daubechies)                      & 0.888      & 0.068     & {0.922}      & {0.040}     \\
          Ours (coiflet)                     & 0.886      & {0.067}     & 0.916      & 0.046     \\
          Ours (haar)                     & 0.880      & 0.108     & 0.911      & 0.070     \\
          Ours (symlet)                     & 0.885      & 0.106     & 0.911      & 0.069     \\
          \midrule
          \multicolumn{5}{l}{\textbf{Complex-valued Adapters}} \\ \midrule
          Ours (Symmetric-b) & {0.892}      & {0.067}     & 0.917      & 0.045     \\
          Ours (Symmetric-a)  & {0.893}   & {0.066}     & 0.912      & 0.046     \\
          \midrule
    \multicolumn{5}{c}{SAM2 as backbone}\\
    \midrule
              \multicolumn{5}{l}{\textbf{Real-valued Adapters}} \\ 
    \midrule
          Ours (daubechies)                      & {0.896}     & \textbf{0.051}     & 0.923      & \textbf{0.036}     \\
          Ours (coiflet)                     & 0.893      & \textbf{0.051}     & 0.924      & 0.039     \\
          Ours (haar)                     & 0.894      & \textbf{0.051}     & \underline{0.925}      & \underline{0.037}     \\
          Ours (symlet)                     & 0.893      & \textbf{0.051}     & 0.924      & 0.038 \\
          \midrule
          \multicolumn{5}{l}{\textbf{Complex-valued Adapters}} \\ 
          \midrule
          Ours (Symmetric-b)     & \textbf{0.907}    &  \underline{0.052}       & \textbf{0.928} & \textbf{0.036}     \\
          Ours (Symmetric-a)     & \underline{0.902}    & 0.056        & \underline{0.925} & 0.039   \\
          \midrule \bottomrule
        \end{tabular}
       
    }
\end{table*}

==> Tables/shadow.tex <==
\begin{table*}[h]
\centering    
        \caption{Comparison with state-of-the-art approaches on shadow detection. The best result is shown in \textbf{bold}, and the second best is \underline{underlined}.}
        \label{tab:shadow}
        \setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1}
        \resizebox{.5\linewidth}{!}{
        \begin{tabular}{lc|c}
        \toprule
        \multirow{2}{*}{Method} & ISTD & SBU \\
                                & BER $\downarrow$   & BER $\downarrow$ \\ \midrule
         DSD$^{(2019)}$\cite{DBLP:conf/cvpr/ZhengQCL19}              & 2.17      & 3.45    \\
         FDRNet$^{(2021)}$ \cite{DBLP:conf/iccv/Zhu0KL21}          & 1.55      & 3.04    \\
         MTMT$^{(2020)}$\cite{DBLP:conf/cvpr/Chen0WW0H20}             & 1.72      & 3.15    \\
         EVP$^{(2023)}$\cite{DBLP:conf/cvpr/LiuSPC23}              & 1.35      & 4.31    \\
         Sam-Adapter$^{(2023)}$\cite{chen2023sam}      & 1.43      & -       \\ 
         Sam2-Adapter$^{(2024)}$\cite{chen2024sam2adapterevaluatingadapting}     & 1.43      & -       \\
    \midrule
    \multicolumn{3}{c}{SAM as backbone} \\ 
    \midrule
    \multicolumn{3}{l}{\textbf{Real-valued Adapters}} \\ 
    \midrule
         Ours (daubechies)            & {1.24} & \textbf{2.93}        \\ 
         Ours (coiflet)            & 1.24 & 3.01        \\
         Ours (haar)                & \underline{1.01} & {3.00}       \\
         Ours (symlet)                 & {1.04} & 3.07        \\
                   \midrule
          \multicolumn{3}{l}{\textbf{Complex-valued Adapters}} \\ \midrule
          Ours (Symmetric-b)         & 1.09      & 3.06     \\
          Ours (Symmetric-a)         & 1.15      & 3.06     \\
          \midrule 
          \multicolumn{3}{c}{SAM2 as backbone} \\ 
    \midrule
          \multicolumn{3}{l}{\textbf{Real-valued Adapters}} \\ 
          \midrule
         Ours (daubechies)            & 1.91 & {3.04}        \\ 
         Ours (coiflet)            & 1.24 & 5.28        \\
         Ours (haar)                & \textbf{0.92} & \underline{2.99}       \\
         Ours (symlet)                 & {1.22} & 3.77        \\
             \midrule
          \multicolumn{3}{l}{\textbf{Complex-valued Adapters}} \\ 
          \midrule
          Ours (Symmetric-b)  & 2.60 & 4.43       \\
          Ours (Symmetric-a)  & 1.32 & 4.32       \\
        \bottomrule
        \end{tabular}
        
    }
\end{table*}

==> Tables/sota.tex <==
%\begin{table}[]
%\centering
%\begin{tabular}{lcccc}
%\toprule
%\multirow{2}{*}{Method} & \multicolumn{2}{c}{DUT} & \multicolumn{2}{c}{CUHK} \\
%                        & $\mathcal{S}_m \uparrow$    & $\mathcal{E}_\phi \uparrow$   & $\mathcal{S}_m \uparrow$   & $\mathcal{E}_\phi \uparrow$ \\ \midrule
%                        &       &      &       &      \\
%                        &       &      &       &      \\
%                        &       &      &       &      \\
%                        &       &      &       &      \\
%                        &       &      &       &      \\
%                        &       &      &       &      \\
%                        &       &      &       &      \\
%                        &       &      &       &      \\
%                        &       &      &       &      \\ \bottomrule
%\end{tabular}
%\end{table}


\begin{table*}
\centering
    \resizebox{\linewidth}{!}{
    \begin{minipage}{\columnwidth}
      \caption{Comparison with state-of-the-art approaches on defocus blur detection. The best result is shown in \textbf{bold}, and the second best is \underline{underlined}.}
      \centering
        \begin{tabular}{lcc|cc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c|}{DUT} & \multicolumn{2}{c}{CUHK} \\
                                & $\mathcal{F}_{\beta} \uparrow$    & $\mathcal{M} \downarrow$   & $\mathcal{F}_{\beta} \uparrow$    & $\mathcal{M} \downarrow$ \\ \midrule
          DeFusionNet$^{(2019)}$\cite{DBLP:conf/cvpr/TangZLWZ19}                      & 0.823      & 0.118     & 0.818      & 0.117     \\
          BTBNet$^{(2018)}$\cite{DBLP:conf/cvpr/ZhaoZ0L18}                      & 0.827      & 0.138     & 0.889      & 0.082     \\
          CENet$^{(2019)}$\cite{DBLP:conf/cvpr/ZhaoZLL19}                      & 0.817      & 0.135     & 0.906      & 0.059     \\
          DAD$^{(2021)}$ \cite{DBLP:conf/cvpr/ZhaoSL21}                     & 0.794      & 0.153     & 0.884      & 0.079     \\
          EFENet$^{(2021)}$\cite{DBLP:journals/tip/ZhaoHHL21}                      & 0.854      & 0.094     & 0.914      & 0.053     \\
          EVP$^{(2023)}$\cite{DBLP:conf/cvpr/LiuSPC23}                      & 0.890      & \underline{0.068}     & \textbf{0.928}      & \underline{0.045}     \\ 
    \midrule
    \multicolumn{5}{l}{\textbf{Real-valued Adapters}} \\ 
    \midrule
          Ours (daubechies)                      & 0.888      & 0.068     & \underline{0.922}      & \textbf{0.040}     \\
          Ours (coiflet)                     & 0.886      & \underline{0.067}     & 0.916      & 0.046     \\
          Ours (haar)                     & 0.880      & 0.108     & 0.911      & 0.070     \\
          Ours (symlet)                     & 0.885      & 0.106     & 0.911      & 0.069     \\
          \midrule
          \multicolumn{5}{l}{\textbf{Complex-valued Adapters}} \\ \midrule
          Ours (Symmetric-b) & \underline{0.892}      & \underline{0.067}     & 0.917      & 0.045     \\
          Ours (Symmetric-a)  & \textbf{0.893}   & \textbf{0.066}     & 0.912      & 0.046     \\
          \midrule \bottomrule
        \end{tabular}
        \label{tab:blur}
    \end{minipage}%
    \hspace{10pt}
    \begin{minipage}{\columnwidth}
      \centering
        \caption{Comparison with state-of-the-art approaches on shadow detection. The best result is shown in \textbf{bold}, and the second best is \underline{underlined}.}
        \begin{tabular}{lc|c}
        \toprule
        \multirow{2}{*}{Method} & ISTD & SBU \\
                                & BER $\downarrow$   & BER $\downarrow$ \\ \midrule
      %   Stacked CNN$^{(2016)}$\cite{DBLP:conf/eccv/VicenteHYHS16}      & 8.60      &  -      \\
      %   BDRAR$^{(2018)}$\cite{DBLP:conf/eccv/ZhuDHFXQH18}            & 2.69      & 3.89    \\
     %    DSC$^{(2018)}$\cite{DBLP:conf/cvpr/Hu0F0H18}              & 3.42      & 5.59    \\
         DSD$^{(2019)}$\cite{DBLP:conf/cvpr/ZhengQCL19}              & 2.17      & 3.45    \\
         FDRNet$^{(2021)}$ \cite{DBLP:conf/iccv/Zhu0KL21}          & 1.55      & 3.04    \\
         MTMT$^{(2020)}$\cite{DBLP:conf/cvpr/Chen0WW0H20}             & 1.72      & 3.15    \\
         EVP$^{(2023)}$\cite{DBLP:conf/cvpr/LiuSPC23}              & 1.35      & 4.31    \\
         Sam-Adapter$^{(2023)}$\cite{chen2023sam}      & 1.43      & -       \\ 
         Sam2-Adapter$^{(2024)}$\cite{chen2024sam2adapterevaluatingadapting}     & 1.43      & -       \\
    \midrule
    \multicolumn{2}{l}{\textbf{Real-valued Adapters}} \\ 
    \midrule
         Ours (daubechies)            & {1.24} & \textbf{2.93}        \\ 
         Ours (coiflet)            & 1.24 & 3.01        \\
         Ours (haar)                & \textbf{1.01} & \underline{3.00}       \\
         Ours (symlet)                 & \underline{1.04} & 3.07        \\
                   \midrule
          \multicolumn{2}{l}{\textbf{Complex-valued Adapters}} \\ \midrule
          Ours (Symmetric-b)         & -      & -     \\
          Ours (Symmetric-a)         & -      & -     \\
          \midrule 
        \bottomrule
        \end{tabular}
        \label{tab:shadow}
    \end{minipage}
    \hspace{10pt}
    \begin{minipage}{\columnwidth}
      \centering
        \caption{Comparison with existing methods on forgery detection. The best result is shown in \textbf{bold}, and the second best is \underline{underlined}.}
        \begin{tabular}{lcc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c}{IMD20} \\
                                & $\mathcal{F}1 \uparrow$    & AUC $\uparrow$   \\ 
        \midrule
         ManTra$^{(2019)}$\cite{DBLP:conf/cvpr/0001AN19}              & -      & 0.748     \\
         SPAN$^{(2020)}$\cite{DBLP:conf/eccv/HuZJCYN20}                & -      & 0.750         \\
         PSCCNet$^{(2022)}$\cite{liu2022pscc}             & -      & 0.806         \\
         TransForensics$^{(2021)}$\cite{DBLP:conf/iccv/HaoZYXP21}      & -      & 0.848         \\
         ObjectFormer$^{(2022)}$\cite{DBLP:conf/cvpr/WangWCHSLJ22}        & -      & 0.821         \\
         EVP$^{(2023)}$\cite{DBLP:conf/cvpr/LiuSPC23}                 & 0.443  & 0.807         \\ 
    \midrule
    \multicolumn{3}{l}{\textbf{Real-valued Adapters}} \\ 
    \midrule
         Ours (daubechies)               &   {0.539}     & {0.874}     \\ 
         Ours (coiflet)               & \textbf{0.626}       & \underline{0.902}     \\
         Ours (haar)               &  \underline{0.614}      & \textbf{0.903}      \\
         Ours (symlet)               & 0.607       & 0.900     \\
                   \midrule
          \multicolumn{3}{l}{\textbf{Complex-valued Adapters}} \\ \midrule
          Ours (Symmetric-b)           & -      & -     \\
          Ours (Symmetric-a)         & -      & -     \\
          \midrule 
         \bottomrule
        \end{tabular}
        \label{tab:forgery}
    \end{minipage} 
    }
\end{table*}

==> sec/6_supple.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary

\section{Additional Results}

\subsection{Quantitative Results}
\label{sec:quant}
As mentioned in the main manuscript, we provide quantitative results of SAMWave with SAM2 as the backbone for defocus blur detection, shadow detection, and forgery detection. We show their quantitative comparison in Tab.~\ref{tab:blur}, \ref{tab:shadow}, and \ref{tab:forgery}, respectively.
In defocus blur and shadow detection, we see performance significant performance gain across multiple datasets. However, for forgery detection, unlike the SAM backbone, we did not see any improvement over previous methods. Similar to EVP, our method also lags behind task-specific methods.


% \subsection{Qualitative Results}
% \label{sec:qual}
% We also provide qualitative results of camouflaged object detection in Fig.~\ref{fig:cod}.


% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{Images/sam_cod_extra.pdf}
%     \caption{Qualitative results of camouflaged object detection of our method compared with existing methods. As expected, both the SAM-adapter and EVP performed worse than our method. }
%     \label{fig:cod}
% \end{figure*}


\begin{table}[t]
\centering
      \caption{Comparison with state-of-the-art approaches on defocus blur detection for SAM2 backbone. The best result is shown in \textbf{bold}, and the second best is \underline{underlined}.}
      \centering
    \resizebox{0.8\columnwidth}{!}{
        \begin{tabular}{lcc|cc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c|}{DUT} & \multicolumn{2}{c}{CUHK} \\
                                & $\mathcal{F}_{\beta} \uparrow$    & $\mathcal{M} \downarrow$   & $\mathcal{F}_{\beta} \uparrow$    & $\mathcal{M} \downarrow$ \\ \midrule
          DeFusionNet$^{(2019)}$\cite{DBLP:conf/cvpr/TangZLWZ19}                      & 0.823      & 0.118     & 0.818      & 0.117     \\
          BTBNet$^{(2018)}$\cite{DBLP:conf/cvpr/ZhaoZ0L18}                      & 0.827      & 0.138     & 0.889      & 0.082     \\
          CENet$^{(2019)}$\cite{DBLP:conf/cvpr/ZhaoZLL19}                      & 0.817      & 0.135     & 0.906      & 0.059     \\
          DAD$^{(2021)}$ \cite{DBLP:conf/cvpr/ZhaoSL21}                     & 0.794      & 0.153     & 0.884      & 0.079     \\
          EFENet$^{(2021)}$\cite{DBLP:journals/tip/ZhaoHHL21}                      & 0.854      & 0.094     & 0.914      & 0.053     \\
          EVP$^{(2023)}$\cite{DBLP:conf/cvpr/LiuSPC23}                      & {0.890}      & \underline{0.068}     & \textbf{0.928}      & 0.045     \\ 
          \midrule
          \multicolumn{5}{l}{\textbf{Real-valued Adapters}} \\ 
    \midrule
          Ours (daubechies)                      & \textbf{0.896}     & \textbf{0.051}     & 0.923      & \textbf{0.036}     \\
          Ours (coiflet)                     & 0.893      & \textbf{0.051}     & 0.924      & 0.039     \\
          Ours (haar)                     & \underline{0.894}      & \textbf{0.051}     & \underline{0.925}      & \underline{0.037}     \\
          Ours (symlet)                     & 0.893      & \textbf{0.051}     & 0.924      & 0.038 \\
          \midrule
          \multicolumn{5}{l}{\textbf{Complex-valued Adapters}} \\ 
          \midrule
          Ours (Symmetric-b)   & -  &  -   & - & -     \\
          Ours (Symmetric-a)   & -     & -     & 0.911     & 0.053     \\ \midrule
          \bottomrule
        \label{tab:blur}
        \end{tabular}
        }
\end{table}



\begin{table}
      \centering
        \caption{Comparison with state-of-the-art approaches on shadow detection on SAM2 backbone. The best result is shown in \textbf{bold}, and the second best is \underline{underlined}.}
        \resizebox{0.6\columnwidth}{!}{
        \begin{tabular}{lc|c}
        \toprule
        \multirow{2}{*}{Method} & ISTD & SBU \\
                                & BER $\downarrow$   & BER $\downarrow$ \\ \midrule
         Stacked CNN$^{(2016)}$\cite{DBLP:conf/eccv/VicenteHYHS16}      & 8.60      &  -      \\
         BDRAR$^{(2018)}$\cite{DBLP:conf/eccv/ZhuDHFXQH18}            & 2.69      & 3.89    \\
         DSC$^{(2018)}$\cite{DBLP:conf/cvpr/Hu0F0H18}              & 3.42      & 5.59    \\
         DSD$^{(2019)}$\cite{DBLP:conf/cvpr/ZhengQCL19}              & 2.17      & 3.45    \\
         FDRNet$^{(2021)}$ \cite{DBLP:conf/iccv/Zhu0KL21}          & 1.55      & 3.04    \\
         MTMT$^{(2020)}$\cite{DBLP:conf/cvpr/Chen0WW0H20}             & 1.72      & 3.15    \\
         EVP$^{(2023)}$\cite{DBLP:conf/cvpr/LiuSPC23}              & 1.35      & 4.31    \\
         Sam-Adapter$^{(2023)}$\cite{chen2023sam}      & 1.43      & -       \\ 
         Sam2-Adapter$^{(2024)}$\cite{chen2024sam2adapterevaluatingadapting}     & 1.43      & -  \\
    \midrule
          \multicolumn{3}{l}{\textbf{Real-valued Adapters}} \\ 
          \midrule
         Ours (daubechies)            & 1.91 & \underline{3.04}        \\ 
         Ours (coiflet)            & 1.24 & 5.28        \\
         Ours (haar)                & \textbf{0.92} & \textbf{2.99}       \\
         Ours (symlet)                 & \underline{1.22} & 3.77        \\
             \midrule
          \multicolumn{3}{l}{\textbf{Complex-valued Adapters}} \\ 
          \midrule
          Ours (Symmetric-b)  & - & -       \\
          Ours (Symmetric-a)  & 1.32 & 4.32       \\
        \midrule \bottomrule
        \end{tabular}
        }
        \label{tab:shadow}
    \end{table}


\begin{table}
      \centering
        \caption{Comparison with existing methods on forgery detection on SAM2 backbone. The best result is shown in \textbf{bold}, and the second best is \underline{underlined}.}
        \resizebox{0.6\columnwidth}{!}{
        \begin{tabular}{lcc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c}{IMD20} \\
                                & $\mathcal{F}1 \uparrow$    & AUC $\uparrow$   \\ 
        \midrule
         ManTra$^{(2019)}$\cite{DBLP:conf/cvpr/0001AN19}               & -      & 0.748     \\
         SPAN$^{(2020)}$\cite{DBLP:conf/eccv/HuZJCYN20}                & -      & 0.750         \\
         PSCCNet$^{(2022)}$\cite{liu2022pscc}                          & -      & 0.806         \\
         TransForensics$^{(2021)}$\cite{DBLP:conf/iccv/HaoZYXP21}      & -      & \textbf{0.848}         \\
         ObjectFormer$^{(2022)}$\cite{DBLP:conf/cvpr/WangWCHSLJ22}     & -      & \underline{0.821}         \\
         EVP$^{(2023)}$\cite{DBLP:conf/cvpr/LiuSPC23}                  & \textbf{0.443}  & {0.807}         \\ 
     \midrule
         Ours (daubechies)         &   0.132      & 0.500           \\ 
         Ours (coiflet)            &   \underline{0.416}      & 0.658           \\
         Ours (haar)               &  0.131      & 0.499    \\
         Ours (symlet)             &   0.372      & 0.686    \\
         \bottomrule
        \end{tabular}
        }
        \label{tab:forgery}
    \end{table} 
